Co-Attentive Equivariant Neural Networks: Focusing Equivariance On Transformations Co-Occurring In Data

Equivariance is a nice property to have as it produces much more parameter efficient neural architectures and preserves the structure of the input through the feature mapping. Even though some combinations of transformations might never appear (e.g. an upright face with a horizontal nose), current equivariant architectures consider the set of all possible transformations in a transformation group when learning feature representations. Contrarily, the human visual system is able to attend to the set of relevant transformations occurring in the environment and utilizes this information to assist and improve object recognition. Based on this observation, we modify conventional equivariant feature mappings such that they are able to attend to the set of co-occurring transformations in data and generalize this notion to act on groups consisting of multiple symmetries. We show that our proposed co-attentive equivariant neural networks consistently outperform conventional rotation equivariant and rotation & reflection equivariant neural networks on rotated MNIST and CIFAR-10.

==> experiments_overview.tex <==

----------------------------------------------------------
## Experiments
----------------------------------------------------------
Conventions:
alr_nom = Attention learning rate equal to nominal
eqbn = Equivariant BatchNormalization
mult_att = multiplicative attention
wdec = weight decay on attention weights. 

----------------------------------------------------------
1. NIN Variations
----------------------------------------------------------
- CIFAR_model_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1							| 83.81 accuracy | slurm-2705364.out WEIRD!

- CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1						| 84.85 accuracy | local

- CIFAR_model_dren_NIN_x4_optim_sgd_lr_0.01_wd_0.0001_seed_1 						| 85.56 accuracy | slurm-2700402.out

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 83.97 accuracy | slurm-2699893.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1	| 83.56 accuracy | slurm-2700439.out
- CIFAR_model_att_dren_NIN_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1 	| 80.99 accuracy | slurm-2700452.out

- CIFAR_model_att_dren_NIN_x4_attmode_local_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1		| ERROR! Cuda out of memory in 1st iteration | slurm-2700457.out
- CIFAR_model_att_dren_NIN_x4_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1	| 85.31 accuracy | slurm-2705352.out  
- CIFAR_model_att_dren_NIN_x4_attmode_global_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 83.57 accuracy | slurm-2700463.out
- CIFAR_model_att_dren_NIN_x4_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1    | 77.83 accuracy | slurm-2700466.out

----------------------------------------------------------
1.2. NIN Variations - Batch Normalization
----------------------------------------------------------
Important: For the variations with Batch Normalization, we initially exclude the regularizer factor from the _softmax_att functions.
Important! --> The batch normalization was NOT equivariant on rotation. This is valid for all the experiments below and those ran before the 31/07/19. 

- CIFAR_model_NIN_batchnorm_optim_sgd_lr_0.01_wd_0.0001_seed_1 								| 87.05 accuracy | local

- CIFAR_model_dren_NIN_batchnorm_optim_sgd_lr_0.01_wd_0.0001_seed_1 							| 87.58 accuracy | slurm-2705635.out
- CIFAR_model_dren_NIN_x4_batchnorm_optim_sgd_lr_0.01_wd_0.0001_seed_1							| 88.23 accuracy | slurm-2705636.out     

- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1			| 86.73 accuracy | slurm-2705631.out 
- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 86.84 accuracy | slurm-2705630.out 

- CIFAR_model_att_dren_NIN_x4_batchnorm_attmode_local_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 86.65 accuracy | slurm-2705619.out
- CIFAR_model_att_dren_NIN_x4_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 86.64 accuracy | slurm-2705618.out 

- CIFAR_model_att_dren_NIN_batchnorm_attmode_global_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1			| 83.67 accuracy | slurm-2706672.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 83.52 accuracy | slurm-2706671.out     

- CIFAR_model_att_dren_NIN_x4_batchnorm_attmode_global_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 83.72 accuracy | slurm-2706669.out
- CIFAR_model_att_dren_NIN_x4_batchnorm_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1		| 81.83 accuracy | slurm-2706670.out 

--------------------------------------------------------------------------

!!! Keep in mind - we are not using any regularization on the weights. Instead, we are increasing their learning rate. This might be unstable. 
+-> Divergence for local and global with lr = 0.1 for:
		CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1
		CIFAR_model_att_dren_NIN_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1

	+-> Following  thing to do: - (1) make learning rate equal and (2) (not yet) add regulatization to the attention weights.
		The global attention fails to converge with lr = 0.1

--------------------------------------------------------------------------

1.3 I know came up with the idea to use a multiplicative attention filter instead of an additive one (more flexibility and actually more senseful)

Important! In all the experiments (up to those with "eq_bn", the batch normalization applied was actually NOT equivariant to rotation)
+--> destroyed the entire network structure

--------------------------------------------------------------------------
- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_mult_att	| accuracy 87.14 | slurm-2766448.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_mult_att    | accuracy 83.77 | slurm-2766529.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_mult_att_absval   | accuracy 84.05 | slurm-2766558.out

- CIFAR_model_dren_NIN_batchnorm_optim_sgd_lr_0.01_wd_0.0001_seed_1_2nd_try 						| accuracy 87.53 | slurm-2780761.out
- CIFAR_model_NIN_batchnorm_optim_sgd_lr_0.01_wd_0.0001_seed_1_2nd_try							| accuracy 87.17 | slurm-2780762.out

- CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1_2nd_try							| accuracy 84.69 | slurm-2783151.out
- CIFAR_model_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1_2nd_try								| accuracy 83.57 | slurm-2783154.out

- CIFAR_model_att_dren_NIN_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_2nd_try		| accuracy 81.54 | slurm-2785416.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_2nd_try		| accuracy 82.9  | slurm-2785432.out

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1				| DIVERGENCE! 	 | slurm-2787011.out
- CIFAR_model_att_dren_NIN_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1			| DIVERGENCE!    | slurm-2787013.out

- CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_1								| accuracy 89.01 | slurm-2787014.out
- CIFAR_model_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_1_2nd_try								| accuracy 89.65 | slurm-2787015.out

- CIFAR_model_att_dren_NIN_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_alr_nom 		| DIVERGENCE!	 | slurm-2787174.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_alr_nom			| LATE DIVERGENCE! slurm-2787175.out

- CIFAR_model_att_dren_NIN_batchnorm_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_alr_nom_N_eqbn | accuracy 33.75 --> unstable training | slurm-2787180.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_alr_nom_N_eqbn  | accuracy 88.11 | slurm-2787181.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_alr_nom_N_eqbn | accuracy 86.02  | slurm-2787182.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_global_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_alr_nom_N_eqbn | accuracy 79.76  | slurm-2787183.out


TODO --> Add regularization to the weigths --> DONE
	 We need to recognize if batchnorm is improved / dmgd via the reg_factor in the attention softmax. --> we need a way to control if use it or not. DONE

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_alr_nom_N_wdec


Added way to compare regularization after softmax and Batch Normalization

IMPORTANT! ALL PREVIOUS EXPERIMENTS WITH ATTENTION WERE WRONG....


----------------------------------------------------------
1.3. EXPERIMENTS WITH REPARED - FULLY EQUIVARIANT NETWORKS
----------------------------------------------------------
W! -> If eq_bn is not in the description, we utilize a normal nn.BatchNorm2d procedure instead of the one we developed.

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_rep			| acc: 84.24	| slurm-2793995.out 
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_rep		| acc: 84.5	| slurm-2794007.out


- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_rep			| acc: 88.67	| slurm-2794010.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_rep		| acc: 88.94	| slurm-2794009.out


- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_rep_nodecycle		| acc: 85.9	| slurm-2795681.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_rep_nodecycle	| acc: 86.02	| slurm-2795683.out


- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_rep_nodecycle		| acc: 89.7	| slurm-2795680.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_rep_nodecycle	| acc: 89.93	| slurm-2795684.out

W -> Experiments with adam lead to bad results (partially, not fully evaluated) and divergence. Interestingly, this just happened in LISA, 
     locally, it did not diverge. Even changing the seed.

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_adam_lr_0.01_wd_0.0001_seed_1_attdecay_rep_nodecycle | DIVERGENCE 	| slurm-2797639.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_adam_lr_0.01_wd_0.0001_seed_251_attdecay_rep_nodecycle | DIVERGENCE | slurm-2797653.out

- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_noattreg_attdecay_rep_nodecycle_eqbn	| acc: 86.82 | slurm-2799943.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_rep_nodecycle_eqbn		| acc: 86.09 | slurm-2799942.out - log DELETED

- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_noattreg_attdecay_rep_nodecycle	| acc: 88.04 | slurm-2801449.out
- CIFAR_model_att_dren_NIN_batchnorm_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_rep_nodecycle		| acc: 87.27 | slurm-2801450.out

_____

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_rep_nodecycle	| acc: 85.93 | slurm-2803582.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_attdecay_rep_nodecycle	| acc: 90.21 | slurm-2803583.out

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_rep_nodecycle			| acc: 89.75 | slurm-2803584.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_rep_nodecycle		| acc: 85.41 | slurm-2803585.out

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_rep				| acc: 85.01 | slurm-2803591.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_rep				| acc: 88.1  | slurm-2803592.out

- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_attdecay_rep			| acc: 90.11 | slurm-2803593.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_rep			| acc: 85.64 | slurm-2803594.out


- CIFAR_model_att_dren_NIN_x4_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_rep_nodecycle	| acc: 85.38 | slurm-2803693.out
- CIFAR_model_att_dren_NIN_x4_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_rep_nodecycle	| acc: 85.72 | slurm-2803595.out

- CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1_nodecycle								| acc: 86.09 | slurm-2805426.out
- CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_1_nodecycle								| acc: 89.86 | slurm-2805427.out

- CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_101_nodecycle								| acc: 89.61 | slurm-2805428.out
- CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_101_nodecycle								| acc: 85.31 | slurm-2805429.out, slurm-2806833.out

-- x4 was not really x4. Check --> Was NOT!
- CIFAR_model_att_dren_NIN_x4_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_nodecycle_160_240_320 | acc: 87.65 | slurm-2806842.out
- CIFAR_model_att_dren_NIN_x4_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_attdecay_nodecycle_160_240_320  | acc: 90.62 | slurm-2806843.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_attdecay_nodecycle_160_240_320     | acc: 90.48 | slurm-2806844.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_nodecycle_160_240_320    | acc: 88.2  | slurm-2806845.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_nodecycle_160_240_320	     | acc: 87.99 | slurm-2806846.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_nodecycle_160_240_320	     | DIVERGENCE | slurm-2806847.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_nodecycle			     | DIVERGENCE | slurm-2808378.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_nodecycle			     | acc: 85.32 | slurm-2808471.out
- CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_nodecycle	     		     | DIVERGENCE | slurm-2808378.out


-- At this point, we changed the attention mechanism again, so that it is equviariant to rotation as well. Hence, if the input is rotated, the attention mechanism will rotate as well. 


CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_nodecycle_eqatt			| acc: 86.45	| slurm-2809083.out
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_eqatt				| acc: 86.74	| slurm-2809084.out
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_eqatt				| acc: 85.93	| slurm-2809085.out
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_eqatt_nodecycle  		| acc: 86.22    | slurm-2809088.out	

CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_attdecay_eqatt_nodecycle		| acc: 89.69	| slurm-2810372.out
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_eqatt_nodecycle			| acc: 90.02	| slurm-2810373.out
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_eqatt				| acc: 89.29	| slurm-2810374.out		
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_attdecay_eqatt				| DIVERGENCE	| slurm-2810375.out

CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_101_attdecay_eqatt_nodecycle_160_240_320	| acc: 88.07	| slurm-2810376.out
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.01_wd_0.0001_seed_1_attdecay_eqatt_nodecycle_160_240_320    	| acc: 88.12	| slurm-2810377.out

CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_1_attdecay_eqatt_nodecycle_160_240_320    | DIVERGENCE | slurm-2810416.out	
CIFAR_model_att_dren_NIN_attmode_local_attmech_softmax_bias_optim_sgd_lr_0.1_wd_0.0001_seed_101_attdecay_eqatt_nodecycle_160_240_320  | acc: 90.67 | slurm-2810417.out

- Experiments searching for the best learning rate scheduling configuration

CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1_160_240_320					| acc: 87.75 | slurm-2810406.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_1_160_240_320					| acc: 90.48 | slurm-2810407.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_101_160_240_320					| acc: 90.38 | slurm-2810408.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_101_160_240_320					| acc: 87.56 | slurm-2810409.out

CIFAR_model_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_101_160_240_320					| acc: 87.42 | slurm-2810411.out
CIFAR_model_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_101_160_240_320						| acc: 90.44 | slurm-2810412.out
CIFAR_model_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_1_160_240_320						| acc: 90.53 | slurm-2810414.out
CIFAR_model_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1_160_240_320						| acc: 87.22 | slurm-2810415.out

CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_101_nodecycle_160_260_320				| acc: 87.53 | slurm-2812706.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1_nodecycle_160_260_320				| acc: 87.1  | slurm-2812707.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_1_nodecycle_160_260_320				| DIVERGENCE | slurm-2812708.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_101_nodecycle_160_260_320				| acc: 90.06 | slurm-2812709.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_101_160_260_320					| acc: 89.79 | slurm-2812710.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.1_wd_0.0001_seed_1_160_260_320					| acc: 89.98 | slurm-2812711.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_1_160_260_320					| acc: 86.84 | slurm-2812712.out
CIFAR_model_dren_NIN_optim_sgd_lr_0.01_wd_0.0001_seed_101_160_260_320					| acc: 87.0  | slurm-2812713.out













































